JeDi: Joint-Image Diffusion Models for Finetuning-Free Personalized Text-to-Image Generation

Personalized text-to-image generation models enable users to create images that depict their individual possessions in diverse scenes, finding applications in various domains. To achieve the personalization capability, existing methods rely on finetuning a text-to-image foundation model on a user's custom dataset, which can be non-trivial for general users, resource-intensive, and time-consuming. Despite attempts to develop finetuning-free methods, their generation quality is much lower compared to their finetuning counterparts. In this paper, we propose Joint-Image Diffusion (\jedi), an effective technique for learning a finetuning-free personalization model. Our key idea is to learn the joint distribution of multiple related text-image pairs that share a common subject. To facilitate learning, we propose a scalable synthetic dataset generation technique. Once trained, our model enables fast and easy personalization at test time by simply using reference images as input during the sampling process. Our approach does not require any expensive optimization process or additional modules and can faithfully preserve the identity represented by any number of reference images. Experimental results show that our model achieves state-of-the-art generation quality, both quantitatively and qualitatively, significantly outperforming both the prior finetuning-based and finetuning-free personalization baselines.

==> figs/attention_vis.tex <==
\begin{figure*}[t]
\begin{center}
\vspace{-10pt}
% \fbox{\rule{0pt}{1.5in} \rule{\linewidth}{0pt}}
\includegraphics[width=\linewidth]{figs/attentionmaps.pdf}\\
\end{center}
\vspace{-15pt}
\caption{\textbf{Visualization of the coupled self-attentions.} 
For each element in the bottom image, the correspondence map (Corr.) shows the connections to the element of the highest attention weight in the top image, with the weight denoted by the transparency of the line. The heatmap visualizes the distribution of the attention weights for the element marked with a red box. We observe that similar regions in different images are co-attended in the coupled self-attention layers.  %\tingchun{I find the caption a bit unclear; for example what is "second image" and what is "first image". Maybe we should put "correspondence map" and "heat map" at the top of the image?}
}
\vspace{-10pt}
\label{fig_attn_vis}
\end{figure*}


==> figs/ours_highres.tex <==
% \begingroup
\setlength{\tabcolsep}{0.5pt}
\renewcommand{\arraystretch}{0.5}
\begin{figure*}[ht!]
    \centering
    \vspace{-10pt}
    \includegraphics[width=\textwidth]{figs/results_zeroshot.pdf}
    % \begin{tabular}{cccc}
    %     \includegraphics[width=0.14\textwidth]{figs/ours_highres_imgs/input1.jpg} &
    %     \includegraphics[width=0.27\textwidth]{figs/ours_highres_imgs/img11.jpg} &
    %     \includegraphics[width=0.27\textwidth]{figs/ours_highres_imgs/img12.jpg} & 
    %     \includegraphics[width=0.27\textwidth]{figs/ours_highres_imgs/img13.jpg} \\
    %     {\centering Input} & {\centering Text 11} & {\centering Text 12} & {\centering Text 13} \\[3mm]

    %     \includegraphics[width=0.14\textwidth]{figs/ours_highres_imgs/input2.jpg} &
    %     \includegraphics[width=0.27\textwidth]{figs/ours_highres_imgs/img21.jpg} &
    %     \includegraphics[width=0.27\textwidth]{figs/ours_highres_imgs/img22.jpg} & 
    %     \includegraphics[width=0.27\textwidth]{figs/ours_highres_imgs/img23.jpg} \\
    %     {\centering Input} & {\centering Text 21} & {\centering Text 22} & {\centering Text 23} \\[3mm]

    %     \includegraphics[width=0.14\textwidth]{figs/ours_highres_imgs/input3.jpg} &
    %     \includegraphics[width=0.27\textwidth]{figs/ours_highres_imgs/img31.jpg} &
    %     \includegraphics[width=0.27\textwidth]{figs/ours_highres_imgs/img32.jpg} & 
    %     \includegraphics[width=0.27\textwidth]{figs/ours_highres_imgs/img33.jpg} \\
    %     {\centering Input} & {\centering Text 31} & {\centering Text 32} & {\centering Text 33} \\

    % \end{tabular}
    \vspace{-5pt}
    \caption{\textbf{Personalized text-to-image generations.} We show the generations obtained by our \jedi model on challenging uncommon input subjects shown in the left column. \jedi accurately preserves the reference image content while being faithful to the text prompt.}
    \vspace{-10pt}
    \label{fig:our_generations_highres}
\end{figure*}
% \endgroup

